Length and Velocity Scales in Protoplanetary Disk Turbulence

In the theory of protoplanetary disk turbulence, a widely adopted \emph{ansatz}, or assumption, is that the turnover frequency of the largest turbulent eddy, $\Omega_L$, is the local Keplerian frequency $\Omega_K$. In terms of the standard dimensionless Shakura-Sunyaev $\alpha$ parameter that quantifies turbulent viscosity or diffusivity, this assumption leads to characteristic length and velocity scales given respectively by $\sqrt{\alpha}H$ and $\sqrt{\alpha}c$, in which $H$ and $c$ are the local gas scale height and sound speed. However, this assumption is not applicable in cases when turbulence is forced numerically or driven by some natural processes such as Vertical Shear Instability. Here we explore the more general case where $\Omega_L\ge\Omega_K$ and show that under these conditions, the characteristic length and velocity scales are respectively $\sqrt{\alpha/R'}H$ and $\sqrt{\alpha R'}c$, where $R'\equiv \Omega_L/\Omega_K$ is twice the Rossby number. It follows that $\alpha=\alphat/R'$, where $\sqrt{\alphat} c$ is the root-mean-square average of the turbulent velocities. Properly allowing for this effect naturally explains the reduced particle scale heights produced in shearing box simulations of particles in forced turbulence, and may help with interpreting recent edge-on disk observations; more general implications for observations are also presented. For $R'>1$ the effective particle Stokes numbers are increased, which has implications for particle collision dynamics and growth, as well as for planetesimal formation.

==> addons.tex <==
%This \sout{revised expression} \wladsez{It's not a revised expression. It's the correct alpha, using velocity correlations, whereas the expression using only vrms is an approximation. I would say this is how to correct an approximate alpha using vrms to the correct expression. Let me think about how to rephrase it.}

%We discuss the implications of this regime further below in section \ref{sec:ansatz_not_true}. 

%picked by the Coriolis force, which, in the absence of other forces, will impose the 

%\sout{Here, we analyze the more general case, lay out a simple new approach, and discuss the implications for disk observations, particle growth and settling, and planetesimal formation.}

%\wladsez{Moved here the last paragraph of the "historical perspective", because it is not actually a historical perspective, it's expanding on the motivation why considering different $\Omega$ is important, because of the Stokes numbers.}

%\subsection{A Historical Perspective}

%\wladsez{This first paragraph is repeated information from the introduction. I think this subsection should be removed and incorporated into a single introduction without subsections.}

%The spatial and temporal evolution of turbulent protoplanetary gas and particle disks is determined by the large-scale effective viscosity and diffusivity of the gas, and the particles in it. For many purposes, it is adequate (and indeed necessary given our limited understanding) to simplify the complex effects of real turbulence into a scalar viscosity $\nu$ and diffusivity $D$. The basic scaling or mixing length approximation for turbulent diffusivity and viscosity is $\left(D, \nu\right) \equiv [L][V_L]$,  where $L$ and $V_L$ are respectively the characteristic length and velocity scales of the turbulence. In this case, $L$  can be identified with the energy injection scale or the energy containing large spatial scale and $V_L$ is the velocity at that scale. \citet{Shakura_Sunyaev_1973}  introduced the widely-used mixing length-like closure model $\nu \equiv \alpha c H$ to incorporate our ignorance about the turbulence into the single parameter $\alpha$, where $c$ is the gas sound speed and $H$ is the gas vertical scale height. In this classic paper\footnote{We note that the first description and application of mixing length theory to disks may be found in \citet{Prendergast_Burbidge_1968}, but an explicit mathematical prescription was not given.}, it was suggested briefly that $L \sim H$ and thus $V_L \sim \alpha c$, indeed with $\alpha$ often taken to be of order unity  %$V_L$  to be an order-unity fraction of $c$ (or some adjustable parameter independent of $\alpha$) 
%\citep{Cameron_1978, Lin_Bodenheimer_1982, Weidenschilling_1984, Morfill_1985, Weidenschilling_Cuzzi_1993}, \REV{given that early works were more focused on accretion disks around compact objects where trans-sonic turbulence used to be widely believed.} 

%\wladsez{How can both $V_L \sim \alpha c$ and $V_L \sim c$ (to order unity) unless $\alpha$ is order unity as well?}\jefsez{in the early work $\alpha$ was often $\sim 1$; 1/3 was a popular choice. Remember the early work came from the black hole community, and sonic turbulence was even widely believed for the nebula. But something went wrong with the wording above and I reworded it. }

%The traditional approximation for turbulent diffusivity and viscosity is $\left(D, \nu_T\right) \equiv [L][V_L] \equiv \alpha c H$, where $L$ and $V_L$ are the characteristic length and velocity scale respectively. $L$ in this case can be asserted as the energy injection scale or the energy containing large spatial scale (the integral scale) and $V_L$ is the velocity at that scale. This formalism of $\alpha$-prescription of viscosity incorporates all of our ignorance into the single parameter $\alpha$ circumventing the ambiguities as to what $L$ and $V_L$ individually are. 

%\orksez{also these include gently varying zonal flows too -- their timescales are too slow to straighten out against the shear -- might need to be mentioned here, maybe.}

%The ansatz, evidently, does not address cases where $\Omega_L > \Omega_K$, which may be the case when turbulence is forced in a box or the naturally occuring turbulence in the nebula through mechanisms, such as Vertical shear instability (VSI) \cite{Nelson_etal_2013}, magnetorotational instability (MRI) \cite{balbus_Hawley_1991} or convective overstability (COV) \cite{Lyra_2014}. Moreover, such situations are not restricted by the coriolis effect arising due the rotation of the nebula. However, whether the ansatz is applicable in such cases is still untested.

%\subsection{Distribution of $\alpha$ for $\Omega_K = \Omega_L$}\label{sec:omegaL=omegaK}

%An independent approach that leads to an estimate for $\alpha$ in rotationally supported flows comes from its posited relationship to a system's turbulent Reynolds stresses \citep[e.g.][]{Stoll_Kley_2014, Nelson_etal_2013} are numerically calculated from actual velocity correlations rather than only their magnitudes. 
%\orksez{The above sentence is both unclear and problematic.  Remember,  the studies that are cited here use the tangential stresses to estimate $\alpha$ based on the SS73 formulation, which *is* a mixing length theory connecting the diffusive coefficient to the Maxwell stresses in *rotationally supported flows*.  So I don't understand what you are trying to say here.  Either restate it or strike it.  I've striken 2 other superflous sentences as well -- either accept these or re-incoporate them into your revised text}
%\sout{This distinction may be worthy of future study.} 
%The ansatz presented here is applicable in problems where the mixing length formalism $(D,\nu_T) = \alpha c H$ is used.

%\begin{equation}
%    (D,\nu_T) \sim LV_L \sim \alpha c_s H \sim \alpha H^2 \Omega_K.
%\end{equation}

%given by $R_0 \equiv \Omega_l/2\Omega_K$ 

%Note that in geophysical fluid dynamics $R_0$ is generally defined as $(V_L/L)/2\Omega_K$.  

%%    (D,\nu_T) \sim LV_L \sim L^2 
%%    \Omega_L \sim R'L^2 \Omega_K = 
%%    \alpha H^2 \Omega_K.

%\orksez{The above is confusing.  Who said that $\tau_{K}$ = 1, did they say it? If so, then why?  This comes out of left field.  Please clarify this one way or the other.}

%\footnote{The careful reader will note that Fig. 6 of \citet{Youdin_Lithwick_2007} does not correctly represent how \citet{Cuzzi_etal_1993} modeled $R'>1.$}


%Hence, the regime $\Omega_L>\Omega_K$ does not change the expression of the scalar turbulent viscosity, but affects the individual scaling for the length and velocity scales by a scaling factor of $\sqrt{R'}$ and $1/\sqrt{R'}$ respectively.
%\orksez{I am assuming that this definition will help clarify the other way people assign $\alpha$ based on the root-mean-square averaged velocity fluctuations in a simulation, ile., $\alpha \sim \delta u^2/c_s^2$.}

%\sout{under the strict assumptions that the largest turbulent eddy is subsonic and the eddy acceleration does not exceed the one from vertical gravity. So, even though theoretically $H$ is the largest possible scale available for subsonic turbulence,} 
%\wladsez{I disagree with this sentence. $H$ is the largest isotropic scale of the turbulence, so if the turbulence reaches the scales of $H$ (through either that scale being unstable, or through inverse cascade, then $H$ will shape the turbulence: it thus has ``bearing" on the turbulence.} However, the (gas) disk scale height $H$ stems from the hydro-static balance by disentangling the gas dynamics from the local turbulence, particularly under the assumptions that the largest turbulent eddies are subsonic and have accelerations small compared to the local gravity.
%\wladsez{What is ``realistic''? And why no bearing? The scale $H$ sets the last isotropic scale of the system. It's a natural scale of the disk.} 

%\wladsez{Not true for the MRI. The MRI generates structures of size $H$.}

%\jefsez{note you only SHOW up to $\sqrt{\alpha}H$ which is still much smaller than a vortex}

%\orksez{Don't forget to include the table of simulations, number of resolution elements and a brief discussion of under-resolved spectral range and comment on whether or not that has any bearing on the estimates for $R'$.}

%The calculation of $R'$ from the turbulent kinetic energy spectra $E(k)$ (see section \ref{sec:omegaL_FA} and figure \ref{fig:cartoon}) only requires identifying the energy at the injection scale, and hence is not sensitive to resolution as long as the injection scale and the energy at that scale can be extracted from the generated spectra. 
%\orksez{Be careful here in your sentence above.  I think we need to have at least some inertial range to be present in order to correctly account for it.  If the dissipation is too close to the injection scale then the actual energy levels achieved at that scale might be a lot lower. A guy like Marcus or Barranco will rain hell on us for this if you are too loose with your language here.  Please fix.}
%In that sense, a resolution half of what has been used here would be sufficient for an accurate calculation of $R'$. However, in section \ref{sec:numericaltest} we present a numerical test of the ansatz presented here by analysing the particle scale heights in turbulent medium. Although scale height for inertial particles is effectively set by the largest eddy, the presence of a few smaller eddies down the inertial range help to capture the overall particle dynamics better. With the current resolution, the the bandwidth of the inertial range spans about three-quarter of a decade.

%\orksez{No need to mention the following here,but keep in mind  that this is all fine and good when energy transfer is purely inertial, but the minute waves (inertial or what not) are present then things get cloudy.  I think in pure rotation the frequency spectrum of waves is only on the scale of $\Omega_K$.  Just keep it in mind, that's all.}

%\textcolor{magenta}{{\it I suggest deleting this and replacing with the short blue text above:} These taken together with  the assumptions of mixing length theory, in which $D_t \sim V_L L$, we further show in Appendix \ref{sec:mixing_length} that indeed it consistently follows that $\alpha = \tilde\alpha/R'$.  In the same Appendix we also show the equivalence between $\alpha$ and $\sqrt{\tilde\alpha}/k_f H$.} 

%For an alternate derivation of the relation between $\alpha$ and $\alphat$ using $E(k)$, see 

%where $v_t$ identifies here with $V_L$ and $\ell$ with $L$.  

%\wladsez{Ok, I'm getting confused now. I already know that $\alpha \sim v_{\rm rms}^2/c_s^2$ is a ``lazy'' alpha, a shortcut valid only for isotropic and incompressible, whereas the actual alpha is  $\alpha \sim \langle \rho \delta v_r \delta_\phi\rangle/\langle \rho c_s^2 \rangle $. Is this paper about pointing out that people shouldn't be overusing lazy alpha?}

\par
 %Indeed, an estimate for $\alpha$ in rotationally supported flows comes from its posited relationship to a system's turbulent Reynolds stresses \citep[e.g., as done for the VSI turbulence,][]{Stoll_Kley_2014, Nelson_etal_2013} are numerically calculated from actual velocity correlations rather than only their magnitudes. 

 %Due to the presence of rotation and stratification in the simulation, an inverse cascade is unavoidable. $k_f=3$, being close to the domain scale, does not leave enough room for an integral scale to set up properly. Hence, we think a forcing at an injection scale reasnably far from 

%We would like to inform the reader that the power law index found in Figure \ref{fig:spectra}b is extremely sensitive to the values of $\tanstress$ obtained form the simulations. The values for the same from the simulations with $k_f=3$ are scattered all over, although with a positive slope. 
%\orksez{The above paragraph is awkward and weird sounding.  What are you trying to say here?  Please clean up.}

%\jefsez{I propose we lift the text from ``Driven turbulence calculations.." all the way through equation 14 into an appendix, saving more than 10 lines and removing some distracting detail from the flow.}
%\textcolor{blue}{We calculate $\alphat$ directly from our code results using the standard practice $\alphat = V_{\rm rms}^2/c^2$, where $V_{\rm rms}$ is a spatial and temporal average of the fluctuating velocity amplitudes (see Appendix for details). This approach captures the form of the original mixing length ansatz and the Reynolds stress approach (section \ref{sec:omegaL=omegaK}). As noted in equation \ref{eqn:alphaspec}, it also captures the form of the spectral approach to $V_L$. As noted in section \ref{sec:spectra}, we assume  $V_L^2 \approx V_{\rm rms}^2$.}  

%For the temporal average in equation \ref{eqn:alpha_gole} we take the spatial averages at $5$ different snapshots at the statistically steady turbulent state. Using this equation is a perfectly reasonable way to calculate $\alpha$ irrespective of whether the ansatz is true or false. According to equation \ref{eqn:d_nu_t_final}, although the length and velocity scales are individually affected by the value of $R'$, the overall scalar turbulent viscosity $(D,\nu_T)$ remains unchanged.

%We calculate $\alphat$ directly from our code results using the standard practice $\alphat = V_{\rm rms}^2/c^2$, where $V_{\rm rms}$ is a spatial and temporal average of the fluctuating velocity amplitudes (see Appendix \ref{sec:alpha_alphat} for details). 

%is independent of the forcing wavenumber and depends only on $f_0$.

%For lower $k_f$, the characteristic length scale $L$ of the system increases accounting for more   




%The calibration is shown by the green dotted line. The figure makes it clear that the values of $\alpha$ obtained in the simulation box for different $f_0$ are independent of the forcing wavenumber $k_f$ (and hence, the forcing length scale). This is not surprising as the gas dynamics and the associated correlation length for the turbulence in the simulation domain is dominated by the largest eddy. As long as the energy injection rate remains unchanged, smaller eddy compensates for the energy injection with a lower turn-over time without changing $\alpha$. 

%\orksez{I'm sorry but the above argument is confusing.  I thought $V_L \sim \tilde \alpha \sim \alpha R'$?.  Are you varying $f_0$ here?  I'm totally lost (sad face).}

%\orksez{Include error bars in the power-law fits. I also think you need only 3 significant digits here.}

%both of which are $\sim 1$. 
%In section \ref{sec:numericaltest} we show through numerical experiments that the vertical settling of inertial particles indeed follows the revised form of $\alpha$ instead of $\Tilde{\alpha}$.

%\textcolor{red}{However, we note that \citet{Nelson_etal_2013} and \citet{Stoll_Kley_2014} obtained their values of $\alpha$ directly from numerical averages of $<v'_r v'_{\phi}>$ rather than from $V^2_{{\rm rms}}$, so they are indeed proper values of $\alpha$ (see section \ref{sec:SS}).}

%Note that, the vertical settling is a part of the nebula dynamics to which the particles react with St$_K$. Vertical diffusion, on the other hand, is a process related to the nebula turbulence, and hence, St$_L$ comes into play. 

%When orbital dynamics in the nebula is considered, the denominator of equation \ref{eqn:scaleheight} projects a quadratic variation in St$_L$ \citep{Youdin_Lithwick_2007}. However, for St$_K \sim 0.1$ and less under nebula conditions, the diffusion is essentially independent of Stokes number and the change in the calculated scale height is negligible \citep{Cuzzi_etal_2001, Carballido_etal_2011}.

%\textcolor{red}{Here I would not use the digression in blue below but just merge something like ``We believe the residual discrepancy of 13-24\% in particle scale height is due to a mass loading effect, which is the subject of a future study" with the discussion in the next paragraph (Lyra and Kuschner..etc..), and shortening that besides, no need to even refer to a figure there.}} 
%\textcolor{blue}{We calculate $R'$  using equation Eq. (\ref{eqn:omegaL}) directly from the KE spectra produced from the simulation data. It can be seen that when particles are present, the values for $R'$ decreases slightly from their gas-only counterpart (see Figure \ref{fig:figure1}(a)). The values of $h$ using $R'$ from the gas only simulations gives $0.07$ and $0.05$ gas scale heights for $k_f=3$ and $6$ respectively. We haven't observed any significant decrease in the energy at the injection scale, however, we have seen that the injection scale shifts towards lower wavenumber in the presence of particles, producing a smaller $R'$ ($\Omega_L \sim k^{3/2}$). We think that this happens due to some interplay of the two flow fields at those large scales along with some form of energy transfer that is yet to be understood.}

%Note that the small difference between the calculated particle scale height and the ones obtained from the simulations can be attributed to the uncertainties in the calculation of $R'$. In the estimation of $R'$ from the turbulent energy spectra, we use the exact value of $k_f$ assigned in the simulation setup. However, as described in section \ref{sec:forcing}, the code implements the forcing at the spectral band around $k_f$. So the actual forcing wavenumbers vary somewhat from the nominal value. With the $k^{-3/2}$ dependence of $\Omega_L$ (equation \ref{eqn:omegaL}), this small variation in $k_f$ can have noticeable effects on $R'$.

%\citet{Lyra_Kuchner_2013} showed that the particle mass loading and back-reaction can alter the vertical distribution of the particles with the mass loading behaving like an extra gravity. Their figure S4 shows that the peak of the distribution is tapered when this effect is included. However, note that in our numerical experiment, the integrated particle-to-gas mass ratio at the midplane ($\epsilon = \rho_p/\rho_g$) is $0.12$ and $0.15$ for $k_f=3$ and $6$ respectively (figure \ref{fig:scaleheight}(d)), too low to impart a significant effect on the scale height. \textcolor{red}{The next sentence is a little redundant with a sentence above ``.. $h$ is different.. clearly indicating .. of the particles."} Furthermore, both simulations in figure \ref{fig:scaleheight} use the same particle parameters and yet have different scale heights, pointing to the fact that the altered scale height stems from the different values of $\alpha$ originating from two different $R'$ at the forcing scales. 

%\textcolor{red}{In this section we show that the particle scale heights actually follow St$_L$, not St$_K$. We present it by a single plot from our series of simulations with vertical gravity and show the differences between estimated scale height by St$_K$ and the actual scale heights observed in the simulations. We also discuss the possible implications for the observations of edge-on disks} \textcolor{blue}{It might be relevant in this section to mention previous work where this distinction was made. For instance, we made a very clear distinction in Cuzzi et al 1993. Also, it may be relevant to briefly comment that the Youdin and Lithwick expression differs from previous work by Cuzzi et al 1993 and Dubrulle et al 1995 only for particles with St $\sim 1$ and larger, while all combinations of realistic nebula turbulence and particle growth suggest that St $\ll 1$ is the rule and the diffusivity is essentially independent of St.  You can look at Carballido et al 2010 to validate this (Carballido et al 2006 also did some settling simulations you should be aware of). So I expect your results will be in excellent agreement with the older expression (you can see this in the YL figures as well, for St $\ll 1$). Also, remember that Youdin and Lithwick failed to show (in their figure 6) how Cuzzi et al 1993 incorporated $R'>1$. Partly as a result of this, their little numerical experiment failed to distinguish between the two models and the only validation of that theory has been by Carballido et al 2010. } 


%\orksez{I'd like to see this clarified more.  A few extra words explaining what was done and concluded will help explain this to the fence-sitters.}


%There are several situations in which the value of $R'$ may be relevant. \textcolor{blue}{Maybe you may want to put this bit up in section \ref{sec:settling}: For one, analyses of edge-on disks have been used to infer values of $\alpha$ based on assumptions of St that are based on nebula growth models and VLA observations \citep{Villenave_etal_2022, Villenave_etal_2023} but if the active turbulence mechanism has $R' >1$, the same particle sizes will correspond to larger St and the observations will tolerate larger values of $\alpha$. A similar argument is less likely to apply to models in which particle radial diffusivity in and around gaps is used to constrain $\alpha$, \textcolor{red}{Debanjan, I know the Dullemond DSHARP paper but maybe you know some other ones that are more recent, where they constrain $\alpha$ from diffusion profiles?} because as noted above, particle diffusivity in the St $\ll 1$ regime is basically independent of St under plausible conditions.} 

%\orksez{I think that these are very good points to raise, but let's also emphasize that the properties of fully resolved VSI turbulence is not known yet.  All those large scale simualtions have been done in which the fastest growing modes are resolved with 10 grid points at most (scale of $\sim H^2/R$).  It's fair to poin this out because it's a serious source of uncertainty.}

%\orksez{How come \citet{Doi_Kataoka_2021,Doi_Kataoka_2023} are not cited here as they are the only ones with a reliable estimate for $\alpha/{\rm St}$ for HD163296. BTW - these 2 studies were incorrectly cited in the discussion of $\delta v/c$ , above so I removed them from there.}

%\textcolor{blue}{NOTE JEFF MOVED THIS PARAGRAPH TO SUBSECTION 3.6 WHERE IT SEEMED TO FIT MUCH BETTER. PLEASE DELETE IT HERE IF YOU AGREE; The model developed in this article is relevant to several kinds of nebula turbulence, such as that driven by vertical shear instability \citep[VSI;][]{Nelson_etal_2013, Flock_etal_2020} or Convective Overstability  \citep[COV;][]{Lyra_2014}. For example, \citet{Stoll_Kley_2014} found that their VSI simulations had $\Omega_L$ significantly higher than $\Omega_K$ (eddy turnover time $\tau_{{\rm eddy}}<1)$. More recently, the energy spectra presented for global VSI simulations in \citet{Flock_etal_2020}  show that energy injection happens around $k\sim 100$ and the stratification induced inverse cascade sets the largest energy containing scale around $k\sim 20$, suggesting that the value of $R'$ may significantly exceed unity. If the disk turbulence is primarily triggered and sustained by such hydrodynamic processes, the method of estimating $\alpha\sim \delta v^2/c^2 (= \alphat)$  will be an over-estimation, whereas values for $\alpha$ from the analyses of edge-on disks will probably be more consistent with the actual level of disk turbulence.} \textcolor{red}{However, we note that \citet{Nelson_etal_2013} and \citet{Stoll_Kley_2014} obtained their values of $\alpha$ directly from numerical averages of $<v'_r v'_{\phi}>$ rather than from $V^2_{{\rm rms}}$, so they are indeed proper values of $\alpha$ (see section \ref{sec:SS}).}

%\REV{ AND I SUGGEST NOT USING THIS RED MATERIAL, PRETTY MUCH ALL OF WHICH GOT MOVED TO THE NEW BLUE APPENDIX I, TO KEEP THE FLOW AND PACE OF SECTION 5 MOVING: Therefore, we conclude that it is necessary to have at least three independent measurements to obtain a more accurate quantitative estimate of $\alpha$ for an observed disk, provided that the local rotation rate and temperature profiles are reasonably known or estimated. If particle sizes are deduced based on the observation's beam size (e.g., as commonly done in ALMA observations), a dependable measurement of the (local) disk mass will result in a reliable estimation of $\rm{St}_K$. Additionally, measuring the root-mean-square velocity ($V_{\text{rms}}$) through line broadening will yield $\tilde\alpha$ according to its identification in Eq. (\ref{def:alphat_sims}). A measurement of the particle scale height $h$ then presents the final piece of information about $\alpha$ as per Eq. (\ref{eqn:scaleheight}), which is reformulated below
%\begin{equation}
%\frac{h^2}{H^2} = 
%\frac{\tilde \alpha}{R'\rm{St}_K(1+{R'}^2\rm{St}_K^2)},
%\label{eqn:Rprime_equation_obs}
%\end{equation}
%where we have used the relationships
%$\alpha\equiv \tilde\alpha/R'$ found in Eq. (\ref{eqn:alpha_alphatilde}) and the definition $\rm{St}_L \equiv 
%R'\rm{St}_K$. Once $R'$ is determined from the solution of Eq. (\ref{eqn:Rprime_equation_obs}), $\alpha$ can be immediately calculated.}

%\REV{In the absence of a reliable disk mass measurement, the best one can do is to estimate the ratio ${\alpha}/{\St_K}$. Given the measured estimates for ${h}/{H}$ and $\tilde{\alpha} \approx {V_{\text{rms}}^2}/{c^2}$, it follows that:
%\begin{equation}\label{eqn:varphi}
%\frac{\alpha}{\St_K} \approx 
%\begin{cases}
%\displaystyle
%\left(\frac{h}{H}\right)^2 \left[1 + \max\left(\St_K^2, \varphi^{-2}\right)\right], & \text{if } \varphi \gg 1, \\
%\displaystyle
%\left(\frac{V_{\text{rms}}}{c}\right)^{\frac{2}{3}}\left(\frac{h}{H}\right)^{\frac{4}{3}}, & \text{if } \varphi \ll 1,
%\end{cases}
%\end{equation}
%where $\varphi \equiv {h^2 c^2}\big/{H^2 V_{\text{rms}}^2}$ is comprised of observed quantities (see Appendix \ref{sec:revised_alphaSt_from_obs} for details). It is evident that \(\varphi\) is the new key parameter controlling the estimate of \(\alpha\). Previous studies have used a formula similar to the one above in the limit \(\varphi \gg 1\) \citep[e.g.,][among others]{Doi_Kataoka_2023, Villenave_etal_2023}, which is not heavily dependent on \(V_{\text{rms}}\). However, if \(\varphi \ll 1\) due to the magnitude of \(V_{\text{rms}}\), the inferred values for \(\alpha\) in disks where \(h/H\) is significantly small may be underestimated as indicated by the formula above. This consideration should be integrated into all subsequent observational interpretations.}

%height will  is needed to  Along this line, it is important to note that, independent measurements of disk mass (or disk surface density to be more specific), $V_{{\rm rms}}$ and the level of particle diffusion, whether by the scale heights from edge-on disk observations and/or particle diffusion at gap edges . 
 
 
 %but if the active turbulence mechanism has $R' >1$, the same particle sizes will correspond to larger St and the observations will tolerate larger values of $\alpha$. A similar argument is less likely to apply to models in which particle radial diffusivity in and around gaps is used to constrain $\alpha$, \textcolor{red}{Debanjan, I know the Dullemond DSHARP paper but maybe you know some other ones that are more recent, where they constrain $\alpha$ from diffusion profiles?} because as noted above, particle diffusivity in the St $\ll 1$ regime is basically independent of St under plausible conditions.

%\subsection{Equivalent Particle Properties: Stokes number \& Coupling}\label{sec:coupling}

%\jefsez{I'm not sure this subsection adds anything. The first sentence is vague and it's not really true that ALL the particle-gas coupling is determined by $St_L$ (ie, not settling and not radial drift). I didn't understand the bit about correlations, either. } In cases of externally forced turbulence by some preassigned prescription, equation \ref{eqn:forcing_term} being one such example, the inertial particles do not behave in the usual manner, and the defining turbulent properties of the particles will change under such conditions. When $\Omega_L>\Omega_K$, the particle-gas coupling will now be determined by St$_L=t_s\Omega_L$ which is greater than St$_K$, and the particles will behave as if their effective size in the gaseous medium is bigger due to the reduced coupling. Apart from that, the effective $\alpha$ and the corresponding diffusion, which the particles now experience will be enhanced due to the increased correlations of the energy containing scales arising from the faster eddy velocities. 






%as we have been envisioning so far. In a protoplanetary disk, the Keplerian rotation and the associated frequency sets a time scale for the system in the form of $1/\Omega_K$. However when turbulence is present within this system with the largest energy containing eddy having a turnover time smaller than that of the local Keplerian, particle dynamics is dominated by the largest eddy turnover time scale $1/\Omega_L$. In terms of the usual Keplerian frequency $\Omega_K$, the particle size is parametrized by the dimensionless number St$_K=t_s\Omega_K$, where $t_s$ is the particle stopping time, the time taken by an inertial particle to lose all its momentum through collisions with the gas molecules. The values of St$_K$ also determines the level of coupling between the gas and the particles. However, under turbulent conditions, the particle dynamics effectively follow a parametrization done with respect to $\Omega_L$ instead of $\Omega_K$. The new Stokes number, also commonly known as the turbulent Stokes number, then can be defined as St$_L=t_s\Omega_L$ which is connected to St$_K$ by St$_L=R'$St$_K$. In the limiting case where $R'=1$, that is the largest eddy turnover time matches that of the local Keplerian, St$_L$ becomes equal to St$_K$.

%In the context of planetesimal formation, a largely open question in the planet formation theory, a recent promising pathway is turbulent concentration where inertial particles are preferentially clustered according to their Stokes number in a turbulent medium. Although there are as yet no actual numerical simulations testing the feasibility of this mechanism in the context and environment of planetesimal formation, recently, some refined but still statistical predictions have emerged showing  that planetesimals can be formed by Turbulent Concentration \citep{Hartlep_etal_2017, Hartlep_Cuzzi_2020}. In these statistical theories, the particle dynamics and their concentration are predicted based on the large eddy Stokes number St$_L$, not St$_K$. Thus, it is important to keep in mind that while comparing the outputs of any future simulations on turbulent concentration with the statistical predictions, the value of $R'$ needs to be determined first following the method outlined in section \ref{sec:omegaL_FA} in order to assess the value of St$_L$ for a proper comparison.



%\textcolor{red}{Discuss the forced simulation cases. Present the spectrum and the corresponding $R_0$ that the simulations produce. Discuss, how the effective \St changes in a forced simulation when scaling is done in terms of largest eddy turnover time in stead of the local $\Omega$. }

%\wladsez{Please don't attack a paper armed only with speculation. If you think \cite{Dullemond_etal_2018} is wrong, the best course of action is to contact Kees, see what he thinks, do the work, and show  (preferably together) that it is wrong.}

%The new ansatz outlined here has  implications for collision velocities (which depend on turbulent intensity) and particle growth. The implications may not exceed the current uncertainty range in turbulent intensity, but as we grow to understand it better, and work harder to connect growth models with actual particle sizes, we will need to be more careful. Generally speaking, someone running a model for particle growth will need to keep in mind the source or technique used to obtain their assumed turbulent intensity, {\it and} a sense of the plausible associated value of $R' =\Omega_L/\Omega_K$. 

%As discussed in section \ref{sec:hd_observation}, a ``true" value we will continue to call $\alpha$ - related to Reynolds stresses - is obtained from a calculation of $<v'_r v'_{\phi}>$ (or perhaps from a measurement of particle layer thickness in some protoplanetary disk). Meanwhile, we will continue to denote by  $\alphat$ a value of turbulent intensity obtained using spectroscopic techniques, or from  a simple model calculation of $V_{{\rm rms}}/c$. 

%Thus, all the particles of some given physical size now couple to larger and faster eddies. 

%In all particle size ranges, the gas fluctuation velocity $V_g=V_L$ also scales the collision velocities. 



%It's a little more tricky here, because if one's turbulent intensity is of the nature of $\alphat$, one simply uses the traditional $V_L=c\sqrt{\alphat}$ from section \ref{sec:omegaL=omegaK}, which has no $R'$ dependence. However if one's turbulent intensity is of the nature of $\alpha$ in the spirit of \citet{Shakura_Sunyaev_1973}, \citep[in the nature of a Reynolds stress, for example from][]{Balbus_Papaloizou_1999, Nelson_etal_2013, Stoll_Kley_2014, Stoll_Kley_2016}, then one must estimate $R'$ and use equation \ref{eqn:velocity} $(V_L=c\sqrt{\alpha R'}$) from section \ref{sec:ansatz_not_true}.  %which, combined with the ${\rm St}_L$ effect, increases the collision velocity by a full factor of $R'$. (equation \ref{eqn:velocity}). 

%So overall, in the important intermediate size range ${\rm St}_{\eta} < {\rm St} < 1$ where most of the action is found, for any given fragmentation or bouncing velocity limit to growth, the maximum modeled particle size will be smaller for a given $\alpha$ when $R'>1$ than in previous studies.

 %Overall then, the collision velocities are now larger by a factor $R'$ for the intermediate regime, and $R'^{1/2}$ in the heavy particle limit. 

%Moreover, collisional outcomes (bouncing, sticking, fragmentation) which determine particle limiting sizes and their ability to participate in SI or TC \citep{Umurhan_etal_2020} depend on a combination of $V_L$ and $St_L$. Changing $R'$ while keeping $\alphat$ constant actually has little effect on collisional outcomes for the most interesting size ranges (see section \ref{sec:collision_growth}), but nature may change that combination in hard to discern ways. In addition, connecting theoretical models that foster planetesimal formation with observed particle sizes in primitive meteorites, if the particle sizes are influenced by turbulent processes, needs to allow for the influence of the local nebula $R'$ as well as $\alpha$.  

%\subsection{Mixing of Solids in Interplanetary particle Particles (IDPs)}

%There are observations of primitive solar system material that contain suggestions of aerodynamical sorting in turbulence. Perhaps the most direct evidence is a series of studies showing that monomer mineral grains in Interplanetary particle Particles (IDPs) of cometary origin are sorted such that the product of their radius and density is constant - the fingerprint of aerodynamic drag in the small particle (Epstein) regime \citep{Wozniakiewicz_etal_2012, Wozniakiewicz_etal_2013}. In a less obvious way, the sizes of individual chondrules in most primitive meteorites share a common, rather narrow size distribution \citep{Friedrich_etal_2015, Simon_etal_2018}. It has been noted that particles with stopping times comparable to the {\it Kolmogorov eddy} timescale $t_{\eta}$ have significantly lower collision speeds with each other than even slightly smaller or larger particles, that may allow them to stick more easily upon collision \citep{Pan_Padoan_2014}. That is, the preferred criterion is given by \citep{Cuzzi_etal_2001, Cuzzi_Hogan_2003, Hartlep_etal_2017}

%\begin{equation}
%1= \rm{St}_{\eta} = (L/\eta)^{2/3} \rm{St}_K = Re^{1/2}\rm{St}_K = (\alpha \frac{\Omega_K H^2}{\nu_m})^{1/2}\rm{St}_K 
%\end{equation}

% where $\nu_m$ is the molecular viscosity. Using the traditional {\it ansatz}, individual chondrules have been found to satisfy this condition in a crude way under inner nebula conditions \citep{Cuzzi_etal_2001}, but in the case of the IDP monomers, much different conditions requiring lower densities and higher $\alpha$ are required \citep{Cuzzi_etal_2017a, Cuzzi_etal_2017b, Hartlep_Cuzzi_2017}. In both cases, a better understanding of local conditions may now also depend on the local value of turbulent $R'$ in their different regions of formation. Moreover, one of the distinguishing properties of the various different chondrite groups is the  mean size of their chondrules \citep[also https://arxiv.org/pdf/1408.6581.pdf]{Friedrich_etal_2015}, which varies by a factor of about 6. If there were a preferred St for particle growth by sticking, different {\it particle sizes} would satisfy it in locations which might differ in their $\rho_g$, $\alpha$, and/or $R'$. 

%\wladsez{So what's new here? The field knows that alpha values from vrms (lazy alpha) are just an approximation. Observations cannot derive but this vrms-based alpha because there’s no resolution to disentangle the velocity correlations. Also, line broadening measures gas velocities, hence viscosity, whereas dust continuum measures grains, hence diffusion. The field knows that Sc can be non-unity, and that diffusion can be anisotropic. Hubert’s group spent a lot of time in the early 2000s measuring the diffusion anisotropy matrix for MRI, for instance. I'm concerned that this particular claim of the paper is unwarranted.}

%The latter are consistently smaller compared to the ones obtained using  velocity information only.  

 %The theory developed here is thus relevant to several kinds of nebula turbulence, such as that driven by vertical shear instability \citep[VSI;][]{Nelson_etal_2013, Flock_etal_2020} or Convective Overstability  \citep[COV;][]{Lyra_2014}. For example, \citet{Stoll_Kley_2014} found that their VSI simulations had $\Omega_L$ significantly higher than $\Omega_L$ (eddy turnover time $\tau_{{\rm eddy}}<1$. More recently, the energy spectra presented for global VSI simulations in \citet{Flock_etal_2020}  show that energy injection happens at a very high wavenumber $(k_f\sim 100)$ and the stratification induced inverse cascade sets the largest energy containing scale around $k_f\sim 20$, suggesting that the value of $R'$ may significantly exceed unity. 


 
%At the end, we would like to emphasize that interpretations of previous modeling results thought to be characterized by certain combinations of $\alpha$ and ${\rm St}_K$, if obtained without consideration of the associated $\Omega_L$, may need to be reevaluated.

%\wladsez{This last paragraph seems unnecessary.}

%\textcolor{red}{Right below is a new Appendix, that I think nails down something we have been unclear about. What do you guys think?}

%We calculate $\alpha$ in the simulation box using a prescription similar to \citet{Gole_etal_2020} as: 
%\begin{equation}\label{eqn:gole_alpha}
%    \alpha = \frac{1}{c^2}\sum_{i=x,y,z}\left(\overline{\langle |\delta v_i(x,y,z,t)|\rangle}\right)^2 
%\end{equation}

%\jefsez{Need to say more here about the difference between wavenumbers as 1/L and as pure numbers.}

%\jefsez{Debanjan will edit this piece. Meanwhile, we have to check carefully to ensure that our $k$ useage is consistent in the paper, even without this new bit. Sometimes it may be normalized and sometimes not!} 

%\jefsez{Well, I took that whole paragraph on TC out for length, you can put it back in if you like. I thought it would be cleaner to just treat the two processes on a par with each other. People should have at least heard of TC by now. I left the original paragraph in the overleaf with a \% sign.}

%How all these factors will manifest in simulations with the possibility of SI included, is a separate investigation by it's own merit and we will soon present the results in a future paper. 

%Another promising pathway for planetesimal formation is turbulent concentration \citep{Toschi_Bodenschatz_2009, Obligado_etal_2014} where inertial particles are preferentially clustered according to their Stokes number in a turbulent medium. Although there are as yet no actual numerical simulations testing the feasibility of this mechanism in the context and environment of planetesimal formation, recently, some refined but still statistical predictions have emerged showing  that planetesimals can be formed by Turbulent Concentration \citep{Hartlep_etal_2017, Hartlep_Cuzzi_2020}. In these statistical theories, the particle dynamics and their concentration are predicted based on the large eddy Stokes number St$_L$, not St$_K$. Thus, it is important to keep in mind that while comparing the outputs of any future simulations on turbulent concentration with the statistical predictions, the value of $R'$ needs to be determined first following the method outlined in section \ref{sec:omegaL_FA} in order to assess the value of St$_L$ for a proper comparison.

Driven turbulence calculations are quantified by an effective ``driving" $\alpha$ parameter.  Following the prescription described in \citet{Gole_etal_2020}, \jefsez{give other refs who used this general metric} we write this control parameter as $\tilde\alpha$ \footnote{We note that  \citet{Gole_etal_2020} write $\tilde\alpha$ as $\alpha_{{\rm drive}}$.} and it is defined as
\begin{equation}
    \tilde\alpha \equiv 
         \frac{1}{c^2}\sum_{i=x,y,z}\left(\overline{\langle |\delta v_i(x,y,z,t)|\rangle}\right)^2.
\end{equation}
%We calculate $\alpha$ in the simulation box using a prescription similar to \citet{Gole_etal_2020} as: 
%\begin{equation}\label{eqn:gole_alpha}
%    \alpha = \frac{1}{c^2}\sum_{i=x,y,z}\left(\overline{\langle |\delta v_i(x,y,z,t)|\rangle}\right)^2 
%\end{equation}
where $c=1$ is the sound speed and $\delta v_i(x,y,z,t) = v_i(x,y,z,t) - \langle v_i\rangle_{xy}(z,t)$ is the velocity fluctuations. Here $\langle .. \rangle$ denotes the spatial average and the overbar denotes the temporal average with the $xy$ subscript being the spatial average over the $xy$ plane. For the temporal average in Eq. (\ref{eqn:alpha_sengupta}) we take the spatial averages at $5$ different snapshots at the statistically steady turbulent state.

Based on the foregoing discussion it follows that we can define and calculate the diffusive $\alpha$ in the simulation box by reference to the driving parameter $\tilde \alpha$ according to: 
\begin{equation}\label{eqn:alpha_sengupta}
    \alpha = \frac{1}{R'c^2}\sum_{i=x,y,z}\left(\overline{\langle |\delta v_i(x,y,z,t)|\rangle}\right)^2 = \frac{\Tilde{\alpha}}{R'}
\end{equation}

%>>>>>Ork's Appendix H>>>>>
\section{Inferring $\alpha/St_K$ from Observations: A Revision}\label{sec:revised_alphaSt_from_obs}
Eq. (\ref{eqn:Rprime_equation_obs}) can be viewed as a cubic equation for $\St_L$,
\begin{equation}
\St_L^3 + \St_L - \varphi^{-1} = 0.
\label{eqn:cubic_StL}
\end{equation}
Where 
\begin{equation}
\varphi \equiv \frac{h^2}{H^2 \tilde \alpha}
\approx 
\frac{h^2 c^2}{H^2 \tilde V_{{\rm rms}}}.
\end{equation}
 Thus, in general then the turbulent Stokes number is a function of the observables $h/H$ and $\tilde\alpha \sim V_{{\rm rms}}^2$, i.e., $\St_L = \St_L(h/H,\tilde\alpha)$.
Thus Eq. (\ref{eqn:Rprime_equation_obs}) may be re-arranged into
\begin{equation}
\frac{\alpha}{\St_K} = 
\frac{h^2}{H^2}\left[1 + \St_L^2\left(\varphi^{-1}\right)\right].
\end{equation}
In the limit where $\varphi \gg 1$ it follows from the limiting form of the cubic Eq. (\ref{eqn:cubic_StL}) that 
$\St_L \rightarrow \varphi$.  But we also observe that physically speaking $\St_L$ should not be less than $\St_K$, thus we instead say that
\begin{equation}
\St_L = {\rm max}\left(\St_K,\varphi^{-1}\right),
\qquad {\rm for} \ \ 
\varphi \gg 1.
\end{equation}
In the other limit where $\varphi \ll 1$ Eq. (\ref{eqn:cubic_StL}) admits the asymptotic form
$\St_L \rightarrow (1/\varphi)^{1/3}$.  For this limit we find
\begin{equation}
\frac{\alpha}{\St_K} \approx
\left(\frac{h}{H}\right)^{4/3} \tilde \alpha^{1/3}
\qquad {\rm for} \ \ 
\varphi \ll 1.
\end{equation}
A summary of this analysis with appropriate replacements made for $\varphi$ in terms of $V_{{\rm rms}}$ is presented in the final expression Eq. (\ref{eqn:varphi}).

{\it I am not sure of this last part, I found it a little opaque and the reference to ``the one above" unclear without going back into the referenced papers which I have not done. Maybe Ork can make it more explicit. Be careful about appearing to solve for the answer in all limits since we are not even approaching the limit $St < alpha$ where $h \sim H$. Note I changed the definition of $\varphi$ below to correspond to the above:} Previous studies have used a formula similar to equation \ref{eqn:varphi} in the limit \(\varphi \ll 1\) \citep[e.g.,][among others]{Doi_Kataoka_2023, Villenave_etal_2023}, which is not heavily dependent on \(V_{\text{rms}}\). However, if \(\varphi \gg 1\) due to the magnitude of \(V_{\text{rms}}\), the inferred values for \(\alpha\) in disks where \(h/H\) is significantly small may be underestimated as indicated by the formula above. 

{\it I would be careful with commands like the following, since we have not really spoken to any observers. Notice that in my development the end product is not $\alpha/St_K$ but something more meaningful.} This consideration should be integrated into all subsequent observational interpretations.

%%%%%%%%%%%%%%>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>>
    


